A Topological Framework for Finite Behavioural Observations and Verification

Formal verification and monitorability are based on finite observations, which allow properties to be verified from finite information about system behaviour. We study such observations through the topologies they generate on spaces of processes. We first consider trace-based topologies and show that finite trace observations on the space of infinite traces induce the Cantor topology, while the topology corresponding to full trace inclusion is the discrete topology. We then move to arbitrary process spaces, where finite trace observations define the observation topology, and show that simulation observations generate a strictly finer topology. Next, we prove a general verification theorem showing that, for any topology generated by finite observations, open sets are exactly the properties verifiable by those observations. We instantiate this result for the observation and simulation topologies, obtaining multi-trace and simulation monitorability as concrete cases. Finally, we examine the effect of replacing simulation with stronger relations, showing that finite-depth bisimulation induces a topology finer than the simulation topology.

==> eptcsdata.tex <==
\providecommand{\firstpage}{13}
\providecommand{\publicationstatus}{G. Bacci, M. Randour (Eds.): Seventeenth\\
International Symposium on Games, Automata, Logics,\\
and Formal Verification (GandALF 2026)\\
EPTCS 454, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.454.3}{10.4204/EPTCS.454.3}}
\pdfoutput=1

